VINNAS: Variational Inference-based Neural Network Architecture Search

In recent years, neural architecture search (NAS) has received intensive scientific and industrial interest due to its capability of finding a neural architecture with high accuracy for various artificial intelligence tasks such as image classification or object detection. In particular, gradient-based NAS approaches have become one of the more popular approaches thanks to their computational efficiency during the search. However, these methods often experience a mode collapse, where the quality of the found architectures is poor due to the algorithm resorting to choosing a single operation type for the entire network, or stagnating at a local minima for various datasets or search spaces. To address these defects, we present a differentiable variational inference-based NAS method for searching sparse convolutional neural networks. Our approach finds the optimal neural architecture by dropping out candidate operations in an over-parameterised supergraph using variational dropout with automatic relevance determination prior, which makes the algorithm gradually remove unnecessary operations and connections without risking mode collapse. The evaluation is conducted through searching two types of convolutional cells that shape the neural network for classifying different image datasets. Our method finds diverse network cells, while showing state-of-the-art accuracy with up to almost 2 times fewer non-zero parameters.

==> comments.tex <==
{\color{red}

I still think you dive quickly into the details in following paragraph without positioning the paper -- it needs to be done in the introduction. I suggest in the following you insert a numbere of paragraphs per bullet points below

In the very first paragraph, you briefly present your hypothesis. You can also add some additional elements / evidence in support of your hypothesis
}
{\color{red} Bayesian neural networks (BNNs) have been initially introduced in...}



{\color{red} In the next paragraph, you argue that NN search is being investigated for point-wise NNs. You can give a vry brief synopsis of main developments in the area of NN search for pointwise networks}


{\color{red} Finally, you insert on paragraph elaborating about your approach. I would construct such paragraph as follows: "In contrast with existing works in NN search for Bayesian NNs, our approach is based on ...[brief description of your approach]  Our approach therefore has several advantages over existing ones [ref] such as... "}

==> discarded.tex <==
\subsection{Concrete Distribution}\label{sec:background_concrete_distribution}

\paragraph{Expected Calibration Error}
We measure the calibration of the found architectures and their sensitivity through expected calibration error (ECE)~\cite{guo2017calibration}. ECE relates confidence with which a network makes predictions to accuracy, thus it measures whether a network is overconfident in its predictions. To compute ECE, the authors propose to discretize the prediction probability interval into a fixed number of bins, and assign each predicted probability to the bin that encompasses it. The calibration error is the difference between the fraction of predictions in the bin that are correct (accuracy) and the mean of the probabilities in the bin (confidence). ECE computes a weighted average of this error across bins as shown in~\eqref{eq:ece}.
\begin{equation}
    ECE = \sum_{b=1}^{B}\frac{n_{B}}{N}\mid \text{accuracy}(b) - \text{confidence}(b) \mid
    \label{eq:ece}
\end{equation}
where $n_b$ is the number of predictions in bin $b$, $N$ is the total number of data points, and accuracy($b$) and confidence($b$) are the accuracy and confidence of bin $b$, respectively. We set $B=10$.

The concrete categorical or the Gumbel-softmax distribution was jointly proposed by Jang \textit{et al.}~\cite{jang2016categorical} and Maddison \textit{et al.}~\cite{maddison2016concrete} and it is a fully reparametrisable continuous relaxation to Categorical distribution that lets us backpropagate the gradient through otherwise discrete distribution. Sampling $N$ dimensional probability vectors $\boldsymbol{n} \in \mathbb{R}^N$ can now be expressed as a deterministic function of its parameters - the probability vector $\boldsymbol{\mu}$ and an external randomness $\eta$ which is sampled through a Gumbel distribution and the density $p(\textbf{n}|\boldsymbol{\mu}, \tau)$ is expressed as in Equation~\ref{eq:concrete_multiple}. 
\begin{align}
    n_i &= \frac{e^{\frac{\log \mu_i + \eta_i}{\tau}}}
    {\sum_j e^{\frac{\log \mu_j + \eta_j}{\tau}}} \nonumber \\
    \eta_i &\sim -\log(-\log(\textrm{Uniform}(0,1))) \nonumber \\
    p(\textbf{n}|\boldsymbol{\mu}, \tau) &= (N-1)!\tau^{N-1} \frac{\prod_{i=1}^{N}\mu_i n^{-\tau - 1}_i}{\left(\sum_{i=1}^{N}\mu_i n^{-\tau}_i\right)^{N}}
     \label{eq:concrete_multiple}
\end{align}
The $\tau \in \mathbb{R}^1$ is a temperature hyperparameter that can be tuned to relax or restrict the distribution's representation to a discrete or a continuous domain. In the limit $\tau \rightarrow 0$ the samples are going to be one-hot vectors similarly to a concrete distribution, while $\tau \rightarrow \infty$ means that $n_i = n_j$. The authors recommend to start with an arbitrary value of $2/3$ for $\tau$ and anneal it during training of the NN that samples through this distribution.

- uncertainty in the weights is complementary in that it captures uncertainty about which neural network is appropriate, leading to regularisation of the weights and model averaging~\cite{blundell2015weight}

The concrete distribution is ideal for considering whether a particular edge or operation in a NN is active or not. During training, start with relatively high temperature $\tau$ and gradually decrease it to resemble sampling from a Categorical distribution. It is necessary to consider this form of approximation, since it is impossible to propagate gradients through a discrete distribution without making an estimate~\cite{bengio2013estimating}.

- CHALLENGE: 
    - Providing prior knowledge about architecture which is the case for every neural network is challenging and it needs to be investigates
    - If we simply decide to use the MAP estimate as the prior we would have a delta function and we are not going to learn anything new 
    - With the current methodology we cannot express our confidence in selecting that particular architecture - no measure of uncertainty 
    
- SOLUTION:
    - Methods borrowed from neural architecture search to perform Bayesian inference not only on the weights of the network but the structure itself to achieve the best performance and hopefully approach the posterior as close as possible 
    - We do this by adopting an approach from differential neural architecture search and searching for weights that decide which operations are going to be eventually performed
    - Others do it simply by replicating the same cell which is uintuitive 
    - Each cell shares the statistical strength of other cells but at the same time enables personalising
    - These cells are then stacked together to create one network
    
    - We are then able to express the uncertainty of the individual weights as well as the operations and the overall architecture 
    
Gradient-based optimisation is typically based on starting with an over-parametrised NN that is gradually pruned or compressed to achieve a trade-off between the model size and the desired objective. This approach became attractive because it reduces the prohibitive computational cost immensely~\cite{deng2019dbsn}.
- Cell based NAS 
    - sequence of cells which have the same internal structure and are separted by upsampling or downsampling modules 
    - Each cell contains sequential nodes that are connected through operations 
    - Differentiable NAS tries to find the strength of these connections by introducing specific parameters representing the strength and then multipying the output to enable backpropagation 
    - Introduce the states inside the cell, relate to hte introduced figures
    
The cell structure is then defined with respect to these parameters that are defined as $\boldsymbol{\beta}= \{\beta_{i,j}^c; 1 \leq i < j , c = 1, \dots, C\}$ where the indices $i,j$ signify the potential connections between states $S$ inside the cell $c$. In a traditional NAS all gating weights $\boldsymbol{\beta}^c$ are all the same for all cells $c$ or split into categories, but their structure is the same among the few categories. The information for the state inside the cell is then a weighted sum of the outputs from the $K$ different operations on $\boldsymbol{S}_{i}^c$. The output of the cell $\boldsymbol{S}_{j}^{c}$ is then a concatenation of all the previous states $\boldsymbol{S}_{i}^j; i<j$. 

\begin{equation}
    \boldsymbol{S}_{i,j}^c = \sum_{k=1}^{K} \boldsymbol{\beta}_{i,j}^{c,k} o_{i,j}^{c,k}(\boldsymbol{S_{i}^{c}},\boldsymbol{w}_{i,j}^{c})
\end{equation}
    - 


The pruning can then be based on the magnitude of the weights, penalty terms or thresholds~\cite{zhou2019bayesnas}. There is usually no proxy model or controller to guide the search, instead the objective $\mathcal{L}$ is formed in such fashion that it can be optimised both with respect to the weights $\boldsymbol{\theta}$ as well as architecture parameters $\boldsymbol{\phi}$ with respect to data $\mathcal{D}$ as
\begin{equation}
    \boldsymbol{\theta^{*},\phi^{*}}=\textrm{arg}\min_{\boldsymbol{\theta, \phi}}\mathbb{E}[\mathcal{L}(\mathcal{D},\boldsymbol{\theta}, \boldsymbol{\phi})]
\end{equation}


- The main point is that the objective needs to be differentiable
In DARTS Liu \textit{et al.}~\cite{liu2018darts} used a softmax function weighted operations to determine which operation should the given node perform


\paragraph{Bayesian learning}

Dikov \textit{et al.}~\cite{dikov2019bayesian} were optimising specifically the BNNs' layer size and network depth through VI, however, the network operations were fixed their performance was not comparable to the current-state-of-the-art. Zhou \textit{et al.}~\cite{zhou2019bayesnas} were jointly learning the parameters and architecture of a BNN through a Laplace approximation that rapidly reduced the search time and they also obtained results that are more comparable to the current state-of-the-art in comparison to Dikov \textit{et al.}. 

By jointly optimising both the parameters and the architecture of a NN via SGD, it is not necessary to introduce any bias in form of a controller that reflects the bias of the author. Note, that since there is no controller, it is not necessary to spend any time training the controller and we can focus completely on traversing the search space. Moreover, it is not necessary to add any metaheuristics, similar to EA, that need to be tuned and the search is unified under one pattern which core is SGD. However, formulating an objective in a tangible way to induce optimisation not only in terms of the weights, but also in terms of architecture parameters is a challenging task. Nevertheless, the frequency of the respective updates to $\boldsymbol{\theta}$ as well as $\boldsymbol{\phi}$ need to be investigated.

- Dikov et al.

- Bayesian method to structure optimisation by treating hyperparameters, such as layer size and network depth as random variables whose parametrised distributions are learnt together with the rest of the network weights

0 They kept the structure the same

The main observations that have been noted in this research area is the importance of (i) weight sharing among architectures to avoid starting from scratch and save computational resources, (ii) transfer learning and transferring the same architecture from a small proxy task to a more challenging task (iii)

Except methods that are based on continuous relaxation of architecture parameters and differentiable search~\cite{xie2018snas, liu2018darts, dikov2019bayesian, zhou2019bayesnas, cai2018proxylessnas, deng2019dbsn, antoran2020variational} the search strategy, based on the searching algorithm, can be later divided into three other categories: (i) reinforcement learning based on an actor-critic framework~\cite{zoph2016neural, pham2018efficient, cai2018efficient, DBLP:journals/corr/ZophVSL17, Schrimpf2018, Zhong2018, Baker2019, Cai} (ii) evolutionary methods based on evolutionary algorithms~\cite{stanley2002evolving, real2017large, xie2017genetic, real2019regularized, yang2019cars}, (iii) Bayesian optimisation based on proxy models~\cite{jin2019auto, fedorov2019sparse} or (iv) gradient based methods. A comprehensive review was made by Elksen \textit{et al.}~\cite{elsken2018neural} and Hu and Yang~\cite{hu2020technical}.

Reinforcement learning use a controller to sample a sequence of operations that then represents their architecture and they gain their reward from the performance on the validation dataset. Evolutionary methods initialize a set of models as a population which they evolve through self-defined mutation and crossover towards better fitness value. Lat but not least, Bayesian optimiztaion tries to find new architectures through a proxy model, usually a Gaussian process~\cite{williams1996gaussian}, that guides the sampling by balancing evaluation and exploration provided by the proxy model. Given an architecture, these methods have to train it for a large number of epochs, and then evaluate its performance or optimize the controller, population or proxy model, which makes the searching stage less efficient~\cite{yang2019cars}.

\subsection{Automatic Relevance Determination}\label{sec:background_ard}

ARD~\cite{mackay1995probable, neal1996bayesian} is used as a principled criterion to determine the number of latent variables
needed to model the data, especially in high-dimensional regimes. The idea consists of using a prior distribution on weights which encourages the weights to be zero, for example for r.v. $x$: $p(x) = \mathcal{N}(x \mid 0, 1)$. ARD was predominantly used in relevance vector machines~\cite{tipping2001sparse} to compute a mask for the support vectors, which resulted in a sparser model in comparison to support vector machines.

- Factorisable Gaussians ~\cite{titsias2014doubly}

Our main contribution ins concerned with regularising the previously deterministic weights by incorporating uncertainty using prior distributions, but not at the global level, but at the cell level by introducing auxiliary parameters $\boldsymbol{\beta}_{c,normal}\in c=1,\ldots, \sum_i^{C_{normal}}C_i$ where $C_i$ is the number of normal cells replicated with specific $\boldsymbol{\beta}_{c,normal}$ and $\boldsymbol{\beta}_{c,reduce}\in c=1,\ldots, C_{reduce}$. We model $\boldsymbol{\beta}$ using a Gaussian prior distribution $p(\boldsymbol{\beta})= \mathcal{N}(0,\boldsymbol{I})$, where $\boldsymbol{I}$ denotes the identity covariance matrix. In Figure~\ref{fig:graphical_model} we sketch the graphical model along with the prior and approximate posterior distributions. 

Our particular structure of the structure parameters forms a mask over the latent variables $\boldsymbol{\alpha}$, which would otherwise select operations for all cells uniformly. The goal of adding this structure to the model is to facilitate the relevance weights to automatically reach distributions peaked around zero, in order to effectively prune the irrelevant operations suggested by the global parameters or otherwise strengthen other ones. Apart from regularisation and model selection the added variable also provides interpretability when using the model after being
successfully inferred, by allowing the user to inspect the relevant latent variables $\boldsymbol{\beta}$ directly.

Nevertheless, inferring the parameters $\boldsymbol{\beta}$ becomes intractable, therefore we introduce an approximate posterior distribution $q(\boldsymbol{\beta}_c \mid \mathcal{D}, \boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c)$ that we optimise through variational inference. 

To stay consistent with research in NAS~\cite{zoph2016neural, real2019regularized, liu2018darts} we follow the search space-space which has been originally formulated by Zoph \textit{et al.}~\cite{DBLP:journals/corr/ZophVSL17}. 
We seek to fill in a pre-determined network structure defined in Figure which consists of two types of cells: \textit{normal cell} and \textit{reduction cell}. A sample cell structure is shown in Figure~\ref{fig:nas_cell}. It contains operations, which are represented as an edge $(i,j)$, while the nodes $S_i$ represent information. Each node $S_i$ is formed by outputs from two operations $o_{k,j}(S_k) + o_{k,i}(S_j); k,j<i$.

However, our search space differs such that, each normal cell in the search space is custom, while sharing the statistical strengths of the other cells through parameters $\boldsymbol{\alpha}=\{\boldsymbol{\alpha}_{reduce}, \boldsymbol{\alpha}_{normal}\}$ for both the normal and the reduce cells. The cells are stacked to create a network. We model the distribution over the parameters through parameters $\boldsymbol{\beta}_i \in \{1, \ldots, N\}$ for the $N$ normal cells and $\boldsymbol{\beta}_i \in\{1, \ldots, R\}$ for the $R$ reduce cells that can be jointly interleaved.

The cells are collection of   The learned cell could either be stacked to form a
convolutional network or recursively connected to form a recurrent network.
A cell is a directed acyclic graph consisting of an ordered sequence of N nodes. Each node x
(i)
is
a latent representation (e.g. a feature map in convolutional networks) and each directed edge (i, j)
is associated with some operation o
(i,j)
that transforms x
(i)
. We assume the cell to have two input
nodes and a single output node. For convolutional cells, the input nodes are defined as the cell outputs
in the previous two layers (Zoph et al., 2018). For recurrent cells, these are defined as the input at
the current step and the state carried from the previous step. The output of the cell is obtained by
applying a reduction operation (e.g. concatenation) to all the intermediate nodes.

The performance degradation is usually at the expense of Bayesian inference which, however, allows us to add all the previously mentioned advantages to the predictive model. The inference is often done on the weights $w$ of the NN which are, under a Bayesian framework, parametrisable random variables~\cite{titsias2014doubly, blundell2015weight}, e.g.: $q(w) = \mathcal{N}(w \mid \mu,\mu^2\lambda)$ with variational parameters $\mu,\lambda$~\cite{molchanov2017variational,kingma2015variational}. Given the high dimensionality of these random variables across the NN, calculating the posterior distribution analytically becomes intractable. 

- utilize the differentiable Gumbel Softmax [22,15] to mimic one-hot encoding. However, the one-hot nature implies an exclusive competition, which risks being exploited by unfair advantages~\cite{chu2019fair}

In this work we argue that the performance degradation is due to a lack of attention to searching the right BNNs architecture for the task at hand. Most of architecture search has been focused on pointwise NNs though highly successful neural architecture search (NAS)~\cite{zoph2016neural} automation. The main NAS techniques cover reinforcement learning, genetic algorithms, Bayesian optimisation or lately more successful differential search in which the architecture is found simply through backpropagation.

Thus, we automatically assume that all the operations and their organisation in the existing pointwise NN architecture are the most suitable ones, given our representation and chosen prior. This defines a strong assumption on the shape of our model which might not hold~\cite{osawa2019practical, neal1996bayesian} and
lead to poorer performance than simply thinking of the weights as scalars.

Therefore, we hypothesise that in order to get better performance of BNNs it is necessary to actively search for their architecture, rather than naively convert pointwise NNs into a Bayesian setting {\color{red} prefer: counterpart than setting}. We propose to model the architecture $\mathcal{A}$ of the BNN itself as a set of additional random variables $\mathcal{A} \Leftarrow \boldsymbol{\beta}\sim q(\boldsymbol{\beta}|\boldsymbol{\theta}_\beta, \boldsymbol{x}, \boldsymbol{y})$ paired with learnable parameters $\boldsymbol{\theta}_\beta$ {\color{red} need to explain what these additional random variables/parameters represent in terms of aarchitecture/elements of architectur}. To navigate through the search space, we borrow and extend methods from one-shot cell-based differentiable neural architecture search (NAS)~\cite{liu2018darts,xie2018snas} and variational inference~\cite{molchanov2016dropout,kingma2015variational,blundell2015weight, kingma2013auto}. We specifically search for a structure that is composed of groups of cells that gather a variety of operations that are then stacked on top of each other. The operations are organised into two types of cells, \textit{normal} organised into $N$ groups and \textit{reduction} organised into $R$ groups, that similarly to cell-based NAS~\cite{DBLP:journals/corr/ZophVSL17, pham2018efficient,xie2018snas,liu2018darts,deng2019dbsn, liu2017hierarchical}, are replicated and then used to construct the complete BNN. In our \textit{Variational Inference-based Bayesian neural network architecture search (VIBNNAS)} model, each cell shares the statistical strength of other cells of the same type through global parameters $\boldsymbol{\alpha}$, but at the same time, enables personalisation by learning cell-specific relevance parameters. The model is shown in Figure~\ref{fig:nas_complete}. We determine the importance of using particular operations through variational dropout~\cite{molchanov2016dropout, molchanov2017variational, kingma2015variational} and imposing automatic relevance determination (ARD)~\cite{mackay1995probable, neal1996bayesian} priors. To encourage traversal through the operations' search space, we formulated an auto-regularising objective that promotes exploration, but at the same time motivates certainty in the selection. We further demonstrate that the algorithm is not only limited to finding BNN architectures, but it can be used to search a pointwise NN architecture. 
